Towards Efficient Hyperdimensional Computing Using Photonics

Over the past few years, silicon photonics-based computing has emerged as a promising alternative to CMOS-based computing for Deep Neural Networks (DNN). Unfortunately, the non-linear operations and the high-precision requirements of DNNs make it extremely challenging to design efficient silicon photonics-based systems for DNN inference and training. Hyperdimensional Computing (HDC) is an emerging, brain-inspired machine learning technique that enjoys several advantages over existing DNNs, including being lightweight, requiring low-precision operands, and being robust to noise introduced by the nonidealities in the hardware. For HDC, computing in-memory (CiM) approaches have been widely used, as CiM reduces the data transfer cost if the operands can fit into the memory. However, inefficient multi-bit operations, high write latency, and low endurance make CiM ill-suited for HDC. On the other hand, the existing electro-photonic DNN accelerators are inefficient for HDC because they are specifically optimized for matrix multiplication in DNNs and consume a lot of power with high-precision data converters. In this paper, we argue that photonic computing and HDC complement each other better than photonic computing and DNNs, or CiM and HDC. We propose PhotoHDC, the first-ever electro-photonic accelerator for HDC training and inference, supporting the basic, record-based, and graph encoding schemes. Evaluating with popular datasets, we show that our accelerator can achieve two to five orders of magnitude lower EDP than the state-of-the-art electro-photonic DNN accelerators for implementing HDC training and inference. PhotoHDC also achieves four orders of magnitude lower energy-delay product than CiM-based accelerators for both HDC training and inference.

==> sections/cover-page.tex <==
%\onecolumn
\section*{Cover Page}
\vspace{-0.05in}
\begin{center}
\revCommon{Common} \quad \quad
\revA{Reviewer A} \quad \quad
\revB{Reviewer B} \quad \quad
\revC{Reviewer C} \quad \quad
\revD{Reviewer D} \quad \quad
\revE{Reviewer E} \quad \quad
\end{center}
\vspace{-0.05in}
We thank the reviewers for their feedback.
We have updated the manuscript based on the reviewers' feedback using the color coding shown above.
Below we provide the responses to the reviewers' questions and the list of updates we made to the paper.

%\justifying
\begin{FlushLeft}
\vspace{-0.05in}
\noindent \revCommon{Common Questions}
\begin{enumerate}[leftmargin=*]
\item \textbf{Architectural novelty:} PhotoHDC executes both HDC training and inference with multiple encoding schemes, each with distinct operations, all within a single accelerator using dedicated efficient datapaths.
This has never been proposed before to the best of our knowledge.
Please see the added writeup in Section~\ref{sec:intro} (contribution 2) and Section~\ref{subsec:background_photonics}.
\item \textbf{DAC-PD connection:} Please see the added explanation with an example in Section~\ref{subsec:dac_opt}
\item \textbf{Advantage of photonics:} Please check the added writeup in Section~\ref{sec:photonics_advantage}
\item \textbf{1-bit vs. muti-bit accuracy in HDC:} Please check the modified sentences in Section \ref{sec:intro} (page 1).
\item \textbf{Dealing with non-idealities of the devices:} Please check the added writeup in Section \ref{sec:photonic_imperfections}
\end{enumerate}

\noindent \revA{Reviewer A}\\
\begin{enumerate}[leftmargin=*]
\item \textbf{Architectural novelty:} Common question 1.\\
\item \textbf{DAC-PD connection:} Common question 2\\
\item \textbf{Wire delay and MZM modulation speed}: Please check the added writeup at the end of Section \ref{subsubsec:latency_estimation}.\\
\item \textbf{Electronic Chip and Photonic Chip integration}: Please check the added Section \ref{subsec:integration}.
\end{enumerate}

\noindent \revB{Reviewer B}\\
\begin{enumerate}[leftmargin=*]
\item \textbf{Comparison of accuracy, number of EO-OE conversions, ADCs, and DACs:} Please check the added Table \ref{tab:eo-oe-comparison} and the write-up in Section \ref{subsec:comp-sota-dnn-accel}.\\
\item \textbf{DAC minimization technique (DAC-PD connection):} Common question 2.\\
\item \textbf{Benefits of photonics when being dependent on EO-OE conversion:} Photonics enables efficient analog multiplication operation at a 5 GHz speed.
The incident optical signals on the PDs generate photocurrents in proportion to the bias voltages, and the photocurrents are accumulated accordingly to complete dot product and bundling.
Only after all the aforementioned operations are done, the photocurrents are converted to voltages with the TIAs.
Both the PDs and the MZMs can be modulated at very high frequencies (more than 10 GHz), which we cannot do with CMOS-based circuits.
Also please check common question 3 where we address the benefits of PhotoHDC over fully electronic solutions.\\
\item \textbf{Acronyms}: Updated.
\item \textbf{1-bit vs. muti-bit accuracy in HDC}: Common question 4.
\end{enumerate}

\noindent \revC{Reviewer C}\\
\begin{enumerate}[leftmargin=*]
\item \textbf{Context where PhotoHDC can be used:} Please check the added writeup in Section \ref{sec:intro} in the paragraph before the contribution list.\\
\item \textbf{Architectural novelty:} Common question 1.\\
\item \textbf{Encoding methods and datasets:} Please see the highlighted columns in Table \ref{tab:best_params}.
For the experiments, we have added the dataset and encoding methods in the figure/table titles and highlighted them. Also, in every first paragraph of the experiments, the datasets and encoding methods are mentioned.\\
\item \textbf{DAC delay advantage only true for traditional encoding training?:} For traditional encoding and inference. Please check the highlighted parts in Section \ref{subsec:dac_opt} and Section \ref{subsec:tdac_analysis}.\\
\item \textbf{Behavioral simulation, non-idealities, MZM/PD controlling latency:} We did not perform a behavioral simulation of the photonic MVM.
Please check common question 5 where we talk about dealing with the device imperfections.\\
\item \textbf{MAP-HDC and normalization:} Correct. Normalization is required and performed at the A/D interface implicitly.\\
\item \textbf{Citations for accuracy:} Added three more citations at the end of Section \ref{subsec:datasets}.\\
\item \textbf{Dataflow algorithms}: It would take quite some space to add the dataflow algorithms for all scenarios. We apologize for not being able to fit those algorithms within the given page limit.
\item \textbf{Consistency in the notations in the background section and the figure}: Updated the notations in Figure \ref{fig:HDCTrainingAndInference}.
\item \textbf{Figure 5 update:} Updated the caption and showed continuity in the figure.
\item \textbf{Set of formulas for dataflow:} Highlighted in Section \ref{subsec:arch_functionality}.

\end{enumerate}

\noindent \revD{Reviewer D}\\
\begin{enumerate}[leftmargin=*]
\item \textbf{Patent circuit demonstrated in practice or simulation?:} We did not perform any behavioral simulation of the circuit.
The individual components that we used were fabricated and they show the feasibility of practical implementation.
Please check common question 5 where we talk about dealing with the device imperfections.\\
\item \textbf{Splitting loss and waveguide loss:} We have included the splitting loss and waveguide loss in our power estimation and updated the results.
Please check the added losses in Section \ref{subsubsec:power_estimation}.
Given that the laser power is not the dominant component, accounting for those losses leads to $\approx$0.66\% increase in the total power consumption.
This does not change any conclusion of our paper.\\
\item \textbf{Imperfect input signals:} Common question 5.\\
\item \textbf{Imperfect PDs:} Common question 5.\\
\item \textbf{Advantage of photonics:} Common question 3.
\end{enumerate}

\noindent \revE{Reviewer E}\\
\begin{enumerate}[leftmargin=*]
\item \textbf{1-bit vs. muti-bit accuracy in HDC:} Common question 4.
\item \textbf{PhotoHDC vs CiM when using low bit precision:} 
We used 5-bit precision for our comparison between PhotoHDC and CiM because we were constrained by the NeuroSim tool's capability.
As we decrease the bit precision, the energy efficiency of both PhotoHDC and CiM improves. 
However, going to lower bit precision decreases HDC accuracy.
At a broader level, we need to find a sweet spot where we balance the bit precision (to achieve the desired accuracy) with energy efficiency.
We expect PhotoHDC to provide us with a better energy-efficiency vs. accuracy tradeoff than CiM.


\item \textbf{Multi-bit RRAM:} In our comparison, we have used 5-bit RRAM cells for the CiM array to perform matrix-vector multiplication in Neurosim.
\end{enumerate}

\end{FlushLeft}
\twocolumn

% \newpage

% \section*{Questions}

% \subsection*{Reviewer C}


% --- Can the authors comment on in what contexts this accelerator is intended to be used? The most common use case for HDC classifiers is in edge computing contexts, which impose significant power constraints and have limited memory. HDC classifiers are typically not competitive with classic ML models when these resource restrictions are removed.

% \textbf{Cansu:} This question asks about the $10^2{-}10^3$ higher power consumption in PhotoHDC compared to CiM. You can talk about the on-chip integration, etc., but it doesn't answer the actual question. 
% Think if you can reduce the power consumption of your design. 
% What are the limitations? 
% Is it common for datacenter/cloud applications to run HDC? If not, it's not very compelling to just say that we target datacenter workloads.

% --- Have the authors performed a behavioral simulation of the photonic MVM described accelerator design? 

% \textbf{Cansu:} No behavioral simulations but there is only one MZM on the optical path. Check if the cited MZM is fabricated or  simulated.
% Do we cite any particular PDs? 

% --- How tightly can the PhotoDetectors and MZM phase delay elements be controlled, and to what extent is this design sensitive to environmental sensitivities or other non-idealities? 

% \textbf{Cansu:} Check the paragraph I wrote about calibration in Section IV-C. 

% --- Has the latency associated with controlling MZM/PD elements been taken into account?

% \textbf{Cansu:} Cite the MZM paper, and explicitly say what modulation rate the paper achieved using that design. Is there a photodetector paper you cite? Point the reviewer to that paper. Is there a maximum modulation rate for photodetectors? Limiting factors? 

% Reviewer D

% --- One of the biggest problems typically when dealing with waveguided photonics is managing loss, which should be significant both in terms of by mm and even more so when a signal is split. I may have missed it since that part is somewhat dense, but I don't see how the stacked loss due to the splitters or the actual distance traveled (which I would expect to be much less than the splitters) is accounted for in the calculation. This seems like it would shift the tradeoff significantly.

% \textbf{Cansu:} In Section IV-A,  the splitter loss is 0.2 dB. In Fig. 4, there are log2(R) splitters cascaded within an optical channel. Do you calculate the loss by 0.2 dB * log2(R)? Or is the cascaded total loss 0.2 dB? Say explicitly how you calculate, I think that's the concern of the reviewer.

% ---Fundamentally, I am not really sure what photonics is buying you here. Classically a photonic interconnect gives you the ability to take long direct or maybe mid-haul paths faster and with less loss. Here though you have broadcast and very short haul (just to the PD). Why use optical at all, why not just broadcast a bit electrically? Then you can buffer and pipeline and there are lots of other things you can do to manage the performance and energy better. Is this not better \hl{given that you have the ability to do the current integration? How this compares directly to an electrical equivalent circuit?} would be really helpful to understand what exactly the optical processing is buying you here -- as of right now it is very confusing that it could be doing that much better.

% \textbf{Cansu:} The reviewer here asks about an electrical equivalent of this circuit. Is it possible to design an analog electrical circuit by using the same current integration idea? Would that look similar to CiM? 
